Inductive logic programming at 30: a new introduction

Inductive logic programming (ILP) is a form of machine learning. The goal of ILP is to induce a hypothesis (a set of logical rules) that generalises training examples. As ILP turns 30, we provide a new introduction to the field. We introduce the necessary logical notation and the main learning settings; describe the building blocks of an ILP system; compare several systems on several dimensions; describe four systems (Aleph, TILDE, ASPAL, and Metagol); highlight key application areas; and, finally, summarise current limitations and directions for future research.

==> figs/aleph.tex <==
\begin{figure}[ht]
	\centering
	\resizebox{\textwidth}{!}{
	\centering
	\begin{tikzpicture}[scale=1]


		\node (top) at (0,0) {\Huge \tw{pos(A):-}};

		\node[below left=5cm of top] (l1) {\Huge \tw{pos(A):- red(A)}};
		\node[below left=5cm of top, right=of l1] (l2) {\Huge \tw{pos(A):- square(A)}};
		\node[below right=5cm of top, right=of l2] (l3) {\Huge \tw{pos(A):- rectangle(A)}};
		\node[below right=5cm of top, right=of l3] (l4) {\Huge \tw{pos(A):- polygon(A)}};

		\draw[-{Latex}, line width=0.05cm, gray] (top.south)--(l1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (top.south)--(l2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (top.south)--(l3.north);
		\draw[-{Latex}, line width=0.05cm, gray] (top.south)--(l4.north);


		\node[below left=5cm of l1] (l1_1) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{square(A).}\\
			\end{tabular}
		};


		\node[below=5cm of l1, right=of l1_1] (l1_2) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{rectangle(A).}\\
			\end{tabular}
		};


		\node[below right=5cm of l1, right=of l1_2] (l1_3) {
			\Huge

			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}
		};

		\node[below right=of l2, right=of l1_3] (l1_4) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{rectangle(A).}\\
			\end{tabular}
		};

		\node[below right=of l3, right=of l1_4] (l1_5) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}
		};


		\node[below right=of l4, right=of l1_5] (l1_6) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{rectangle(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}
		};

		\draw[-{Latex}, line width=0.05cm, gray] (l1.south)--(l1_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1.south)--(l1_2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1.south)--(l1_3.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l2.south)--(l1_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l2.south)--(l1_4.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l2.south)--(l1_5.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l3.south)--(l1_2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l3.south)--(l1_4.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l3.south)--(l1_6.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l4.south)--(l1_3.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l4.south)--(l1_5.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l4.south)--(l1_6.north);




		\node[below left=5cm of l1_4] (l2_1) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{rectangle(A).}\\
			\end{tabular}
		};

		\node[below left=5cm of l1_5] (l2_2) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}
		};

		\node[below left=5cm of l1_6] (l2_3) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{rectangle(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}

		};

		\draw[-{Latex}, line width=0.05cm, gray] (l1_1.south)--(l2_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_2.south)--(l2_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_4.south)--(l2_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_1.south)--(l2_2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_3.south)--(l2_2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_5.south)--(l2_2.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_4.south)--(l2_3.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_5.south)--(l2_3.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l1_6.south)--(l2_3.north);


		\node[below left=5cm of l2_3] (l3_1) {
			\Huge
			\begin{tabular}{l}
				\tw{pos(A):- } \\
				\quad\quad \tw{red(A), } \\
				\quad\quad \tw{square(A), } \\
				\quad\quad \tw{rectangle(A), } \\
				\quad\quad \tw{polygon(A).}\\
			\end{tabular}
		};

		\draw[-{Latex}, line width=0.05cm, gray] (l2_1.south)--(l3_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l2_2.south)--(l3_1.north);
		\draw[-{Latex}, line width=0.05cm, gray] (l2_3.south)--(l3_1.north);


		\node[left=19cm of top,black] {\tw{\Huge Most general hypothesis}};
		\node[left=16cm of l3_1,black] {\tw{\Huge Most specific hypothesis}};


	\end{tikzpicture}
	}
	\caption{Aleph bounds the hypothesis space from above (the most general hypothesis) and below (the most specific hypothesis). Aleph starts the search from the most general hypothesis and specialises it (by adding literals from the bottom clause) until it finds the best hypothesis.}
	\label{fig:sys:aleph}
\end{figure}

==> figs/bongard.tex <==
\begin{figure}[t]
	\centering
	% \Large
	\resizebox{\textwidth}{!}{
	\begin{tikzpicture}[scale=1]
		
		\draw (0,0)--(10,0)--(10,5)--(0,5)--cycle;
		
		\draw (15,0)--(25,0)--(25,5)--(15,5)--cycle;
		
		\draw[blue] (2.5,2.5) circle (1.5);
		\draw[brown] (5,4)--(9,4)--(7,1)--(5,4);
		
		
		\draw[brown] (20,4)--(24,4)--(22,1)--(20,4);
		
		
		
		
		
	\end{tikzpicture}
	}
	\caption{Bongard problems}
	\label{fig:bongard}
\end{figure}

==> figs/ilp.tex <==
\begin{figure}[ht]
	\centering
	% \Large
	\resizebox{\textwidth}{!}{
	\begin{tikzpicture}[scale=1]

		\node[gray] at (-3, 4) [align=left] {\huge \tw{User-provided input}};
		\node[gray] at (29, 4) [align=left] {\huge \tw{Learning output}};

		\node at (-2.5,0) [align=left] {
			\LARGE
			\begin{tabular}{@{}l@{}}
				%\toprule
				\textbf{Examples} \\
				\midrule
				\tw{last([m,a,c,h,i,n,e], e).} \\
				\tw{last([l,e,a,r,n,i,n,g], g).}\\
    			\tw{last([a,l,g,o,r,i,t,m], m).}\\
				%\bottomrule
			\end{tabular}
		};

		\node at (-2,-4) [align=left] {
			\LARGE 
			\begin{tabular}{@{}ll@{}}
				%\toprule
				\multicolumn{2}{l}{\textbf{Background knowledge}} \\
				\midrule
				\tw{empty(A)} & \tw{A} is an empty list \\
				\tw{head(A,B)} & \tw{B} is the head of the list \tw{A} \\
				\tw{tail(A,B)} & \tw{B} is the tail of the list \tw{A} \\
				%\bottomrule
			\end{tabular}

		};

		\draw[-{Latex},gray,line width=0.8mm] (3,-1)--(6.9,-1);
		\draw[-{Latex},gray,line width=0.8mm] (3.8,-4)--(6.9,-4);

		\draw[rounded corners=0.5mm,line width=0.5mm, fill=gray, fill opacity=0.05] (7,1)--(15,1)--(15,-5)--(7,-5)--cycle;

		\node at (8.5,0.5) {\Large \textbf{ILP system}};

		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l1) at (11,-1) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l21) at (9.5,-2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l22) at (11,-2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l23) at (12.5,-2) {};

		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l31) at (11,-3.2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l32) at (10,-3.2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l33) at (12,-3.2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l34) at (9,-3.2) {};
		\node[draw,circle,minimum size=2mm,fill=gray,fill opacity=0.8] (l35) at (13,-3.2) {};
		\node[circle,minimum size=2mm] (l36) at (8,-3.2) {};
		\node[circle,minimum size=2mm] (l37) at (14,-3.2) {};

		\node[circle,minimum size=2mm] (l41) at (14,-4.4) {};
		\node[circle,minimum size=2mm] (l42) at (13,-4.4) {};
		\node[circle,minimum size=2mm] (l43) at (12,-4.4) {};
		\node[circle,minimum size=2mm] (l44) at (11,-4.4) {};
		\node[circle,minimum size=2mm] (l45) at (10,-4.4) {};
		\node[circle,minimum size=2mm] (l46) at (9,-4.4) {};
		\node[circle,minimum size=2mm] (l47) at (8,-4.4) {};

		\draw[-{Latex}] (l1)--(l21);
		\draw[-{Latex}] (l1)--(l22);
		\draw[-{Latex}] (l1)--(l23);
		\draw[-{Latex}] (l22)--(l31);
		\draw[-{Latex}] (l22)--(l32);
		\draw[-{Latex}] (l22)--(l33);
		\draw[-{Latex}] (l21)--(l34);
		\draw[-{Latex}] (l23)--(l35);

		\draw[-] (l21)--(l36);
		\draw[-] (l23)--(l37);
		\draw[-] (l31)--(l44);
		\draw[-] (l31)--(l45);
		\draw[-] (l31)--(l43);
		\draw[-] (l32)--(l46);
		\node[circle] (t1) at (10.5,-3.8) {};
		\draw[-] (l32)--(t1);
		\draw[-] (l34)--(l47);
		\node[circle] (t2) at (9.5,-3.8) {};
		\draw[-] (l34)--(t2);
		\draw[-] (l33)--(l42);
		\node[circle] (t3) at (11.5,-3.8) {};
		\draw[-] (l33)--(t3);
		\draw[-] (l35)--(l41);
		\node[circle] (t4) at (12.5,-3.8) {};
		\draw[-] (l35)--(t4);

		\draw[-{Latex},gray,line width=0.8mm] (15.2,-1)--(18.8,-1);


		\node at (26,-1) [align=left] {
			\LARGE
			\begin{tabular}{@{}l@{}}
			\textbf{Program} \\
			\midrule
			\tw{last(A,B):- tail(A,C),empty(C),head(A,B).}\\
    		\tw{last(A,B):- tail(A,C),last(C,B).}
			\end{tabular}
		};

		\path[-,brown,line width=0.7mm,bend left] (14,2) edge (12.3,-1.4);
		\node at (15,2.8) {\LARGE
		\begin{tabular}{@{}l@{}}
			Search space over programs \\
			\textcolor{gray}{each node in the search tree is a program}
		\end{tabular}
		};

		\path[-,brown,line width=0.3mm,bend right] (9,-2) edge (5.3,-6);
		\node at (5.3, -6.8) {
			\LARGE
			\tw{last(A,B):- tail(A,B).}
		};

		\path[-,brown,line width=0.3mm,bend left] (13.4,-3.3) edge (16,-6);
		\node at (16,-6.8) {
			\LARGE
			\tw{last(A,B):- tail(A,C),empty(C),head(A,B).}
		};





	\end{tikzpicture}
	}
	\caption{An ILP system learns programs from examples and BK.
	The system learns by searching a space of possible programs which are constructed from BK.}
	\label{fig:ilp_pipe}
\end{figure}

==> figs/lattice.tex <==
\begin{figure}[t]
	\centering
	\Huge
	\resizebox{\textwidth}{!}{
	\begin{tikzpicture}[scale=1]

		{
		\Huge
		\node (examples) at (0,-0.5) [align=left] {
			\begin{tabular}{@{}l@{}}
				%\toprule
				\textbf{Modes} \\
				\midrule
				\tw{modeh(1, son(+,-)).} \\
				\tw{modeb(1, male(+)).} \\
				\tw{modeb(1, parent(-,+)).} \\
				\tw{modeb(1, parent(\#,+)).} \\
				\tw{modeb(1, father(-,+)).} \\
				%\bottomrule
			\end{tabular}
		};
		}
		
		\node (l1_1) at (13,-3) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{male(Y).}
			\end{tabular}
		};
		
		
		\node[right=of l1_1] (l1_2) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{father(Y,X).}
			\end{tabular}
		};
		
		
		
		\node[right=of l1_2] (l1_3) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X).}
			\end{tabular}
		};
		
		
		
%		\node[right=of l1_2] (l1_4) {
%			\Huge
%			\begin{tabular}{l}
%				\tw{son(X,Y):-} \\
%				\quad\quad \tw{parent(frank,X).}
%			\end{tabular}
%		};
%		
%		\node[right=of l1_4] (l1_5) {
%			\Huge
%			\begin{tabular}{l}
%				\tw{son(X,Y):-} \\
%				\quad\quad \tw{parent(clair,X).}
%			\end{tabular}
%		};
		
		\node[above=3cm of l1_2] (top) {\tw{son(X,Y).}};
		
		\draw[-{Latex},gray, line width=0.05cm] (top.south)--(l1_1.north);
		\draw[-{Latex},gray, line width=0.05cm] (top.south)--(l1_2.north);
		\draw[-{Latex},gray, line width=0.05cm] (top.south)--(l1_3.north);
%		\draw[-{Latex},gray, line width=0.05cm] (top.south)--(l1_4.north);
%		\draw[-{Latex},gray, line width=0.05cm] (top.south)--(l1_5.north);
		
%		%fake nodes
%		\node[below=1cm of l1_4] (f1) {};
%		\draw[-,gray, line width=0.05cm] (l1_4.south)--(f1.north);
%		\node[below left=0.5cm of l1_4] (f2) {};
%		\draw[-,gray, line width=0.05cm] (l1_4.south)--(f2.north);
%		\node[below=1cm of l1_5] (f3) {};
%		\draw[-,gray, line width=0.05cm] (l1_5.south)--(f3.north);
%		\node[below left=1cm of l1_5] (f4) {};
%		\draw[-,gray, line width=0.05cm] (l1_5.south)--(f4.north);

		\node[below=5cm of l1_2] (l2_center) {
			\tw{...}
		};
		
		
		\node[left=of l2_center] (l2_1) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{male(X).}
			\end{tabular}
		};
		
		
		\node[left=of l2_1] (l2_3) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(Y).}
			\end{tabular}
		};
		
		
		

		
		
		
	
		\node[left=of l2_3] (l2_5) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(X).}
			\end{tabular}
		};
		
		
		
		
		\node[right=of l2_center] (l2_2) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{male(Y).}
			\end{tabular}
		};
		
		
		\node[right=of l2_2] (l2_4) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{father(Y,X).}
			\end{tabular}
		};
		
		\node[right=of l2_4] (l2_6) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{parent(Y,X).} \\
			\end{tabular}
		};
		
		\draw[-{Latex},gray, line width=0.05cm] (l1_1.south)--(l2_1.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_1.south)--(l2_4.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_2.south)--(l2_3.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_2.south)--(l2_5.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_2.south)--(l2_4.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_3.south)--(l2_2.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_3.south)--(l2_4.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_3.south)--(l2_6.north);
		\draw[-{Latex},gray, line width=0.05cm] (l1_3.south)--(l2_1.north);

		

		
		\node[below=7cm of l2_center] (l3_center) {
			\Huge
			\begin{tabular}{l}
				\tw{...}
			\end{tabular}
		};
		
		
		
				
		
		
		\node[left=of l3_center] (l3_2) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(Y).}
			\end{tabular}
		};
		
		
		
		\node[right=of l3_center] (l3_6) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{male(Y),} \\
			\end{tabular}
		};
		
		\node[right=of l3_6] (l3_8) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{male(X),} \\
			\end{tabular}
		};
		
		
		\node[right=of l3_8] (l3_4) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{father(Y,X).} \\
			\end{tabular}
		};
				
		
	
		
		\node[left=of l3_2] (l3_1) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(X).}
			\end{tabular}
		};
		
		
		\draw[-{Latex},gray,  line width=0.05cm] (l2_5.south)--(l3_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_3.south)--(l3_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_1.south)--(l3_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_2.south)--(l3_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_4.south)--(l3_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_4.south)--(l3_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_4.south)--(l3_4.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_6.south)--(l3_6.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l2_6.south)--(l3_8.north);
		
		\node[below=7cm of l3_center] (lm_center) {\Huge \tw{...}};
		
		\node[right=8cm of lm_center] (lm1_center) {};
		
		
		\node[right=of lm1_center] (lm_1) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(X).}
			\end{tabular}	
		};
		
		
		\node[right=of lm_1] (lm_2) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(claire,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(Y).}
			\end{tabular}	
		};
		
		
		\node[below=8cm of lm_center] (l4_center) {
			\Huge
			\tw{...}
		};
		
		\draw[-{Latex},gray,  line width=0.05cm] (l3_4.south)--(lm_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_4.south)--(lm_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_2.south)--(lm_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_1.south)--(lm_1.north);
		
		
		
		\node[left=of l4_center] (l4_1) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(X),} \\
				\quad\quad \tw{parent(claire,X).}\\
			\end{tabular}	
		};

		
		
		
		
		
		
		\node[right=of l4_center] (l4_2) {
			\Huge
			\begin{tabular}{l}
				\tw{son(X,Y):-} \\
				\quad\quad \tw{parent(Y,X),} \\
				\quad\quad \tw{father(Y,X),} \\
				\quad\quad \tw{male(Y),} \\
				\quad\quad \tw{parent(claire,X),} 
			\end{tabular}	
		};
		
		
		\draw[-{Latex},gray,  line width=0.05cm] (l3_2.south)--(l4_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_1.south)--(l4_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_6.south)--(l4_2.north);
		\draw[-{Latex},gray,  line width=0.05cm] (l3_8.south)--(l4_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (lm_1.south)--(l4_1.north);
		\draw[-{Latex},gray,  line width=0.05cm] (lm_2.south)--(l4_2.north);
		


		

	\end{tikzpicture}
	}
	\caption{The generality relation orders the hypothesis space into a lattice (an arrow connects a hypothesis with its specialisation). The hypothesis space is built from the modes and only shown partially (\tw{\#} indicates that a constant needs to be used as an argument; only \tw{claire} is used as a constant here). The most general hypothesis sits on the top of the lattice, while the most specific hypotheses are at the bottom. The \textit{top-down} lattice traversal starts at the top, with the most general hypothesis, and specialises it moving downwards through the lattice. The \textit{bottom-up} traversal starts at the bottom, with the most specific  hypothesis, and generalises it moving upwards through the lattice.}
	\label{fig:lattice}
\end{figure}

==> figs/tilde.tex <==
\begin{figure}[t]
	\centering
	\Large
	\resizebox{\textwidth}{!}{
	\begin{tikzpicture}[scale=1]

		\node (top) at (0,0) {\huge \tw{worn(X)}};

		\node[below left=3cm of top] (left_branch) {\huge \tw{irreplaceable(X)}};

		\node[draw, below right=3cm of top] (right_branch) {\huge \tw{ok}};

		\node[draw,below left=3cm of left_branch] (left_branch_2) {\huge \tw{sendback}};

		\node[draw, below right=3cm of left_branch] (right_branch_2) {\huge \tw{fix}};

		\draw[-] (top)--(left_branch);
		\draw[-] (top)--(right_branch);
		\draw[-] (left_branch)--(left_branch_2);
		\draw[-] (left_branch)--(right_branch_2);


		\node[left=7cm of left_branch] {
			\huge
			\begin{tabular}{l}
				\tw{class(X,sendback) :- worn(X), irreplaceable(X), !.} \\
				\tw{class(X,fix) :- worn(X), !.} \\
				\tw{class(X,ok).}
			\end{tabular}
		};






	\end{tikzpicture}
	}
	\caption{TILDE learns tree-shaped (normal) programs. Clauses in the program correspond to paths along the tree.}
	\label{fig:sys:tilde}
\end{figure}
